Sparse Vicious Attacks on Graph Neural Networks

Graph Neural Networks (GNNs) have proven to be successful in several predictive modeling tasks for graph-structured data. Amongst those tasks, link prediction is one of the fundamental problems for many real-world applications, such as recommender systems. However, GNNs are not immune to adversarial attacks, i.e., carefully crafted malicious examples that are designed to fool the predictive model. In this work, we focus on a specific, white-box attack to GNN-based link prediction models, where a malicious node aims to appear in the list of recommended nodes for a given target victim. To achieve this goal, the attacker node may also count on the cooperation of other existing peers that it directly controls, namely on the ability to inject a number of ``vicious'' nodes in the network. Specifically, all these malicious nodes can add new edges or remove existing ones, thereby perturbing the original graph. Thus, we propose SAVAGE, a novel framework and a method to mount this type of link prediction attacks. SAVAGE formulates the adversary's goal as an optimization task, striking the balance between the effectiveness of the attack and the sparsity of malicious resources required. Extensive experiments conducted on real-world and synthetic datasets demonstrate that adversarial attacks implemented through SAVAGE indeed achieve high attack success rate yet using a small amount of vicious nodes. Finally, despite those attacks require full knowledge of the target model, we show that they are successfully transferable to other black-box methods for link prediction.

==> AAAI 2023 SAVAGE --_ ARXIV/macros.tex <==
\newcommand{\Prob}{\mathbb{P}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\Z}{\mathbb{Z}}
\newcommand{\E}{\mathbb{E}}
\newcommand{\insta}{\bm{x}}
\newcommand{\X}{X}
\newcommand{\G}{\mathcal{G}}
\newcommand{\advG}{\widetilde{\G}} %^{\text{adv}}
\newcommand{\Gobs}{\G^{\text{obs}}}
\newcommand{\V}{\mathcal{V}}
\newcommand{\Vnew}{\V^{\text{new}}}
\newcommand{\Vadv}{\V^{\text{adv}}}
\newcommand{\edges}{\mathcal{E}}
\newcommand{\edgesnew}{\edges^{\text{new}}}
\newcommand{\edgesobs}{\edges^{\text{obs}}}
\newcommand{\edgesadv}{\edges^{\text{adv}}}
\newcommand{\graph}{\G=(\V,\edges)}
\newcommand{\neigh}{\mathcal{N}}
\newcommand{\adjM}{A}
\newcommand{\advadjM}{\widetilde{A}}
\newcommand{\adjMij}{{A}_{i,j}}
\newcommand{\dataset}{\mathcal{D}}
\newcommand{\train}{\dataset_{\text{train}}}
\newcommand{\test}{\dataset_{\text{test}}}
\newcommand{\features}{\mathcal{X}}
\newcommand{\labels}{\mathcal{Y}}
\newcommand{\hypspace}{\mathcal{H}}
\newcommand{\params}{\bm{\theta}}
\newcommand{\w}{\bm{\omega}}
\newcommand{\h}{\bm{h}}
\newcommand{\advh}{\widetilde{\bm{h}}}
\newcommand{\hyp}{h_{\params}}
\newcommand{\gnn}{g(\adjM, \X; \W)}
\newcommand{\model}{h^*}
\newcommand{\loss}{\ell}
\newcommand{\ladv}{\ell_{\text{adv}}}
\newcommand{\ldist}{\ell_{\text{dist}}}
\newcommand{\lnew}{\ell_{\text{new}}}
\newcommand{\Loss}{\mathcal{L}}
\newcommand{\savag}{\text{SAVAGE}}


\newcommand{\gabri}[1]{\todo[inline,color=BlueGreen!60]{{\bf Gabri:} #1}}
\newcommand{\fabri}[1]{\todo[inline,color=RedOrange!60]{{\bf Fabri:} #1}}
\newcommand{\ema}[1]{\todo[inline,color=ForestGreen!60]{{\bf Ema:} #1}}
\newcommand{\gio}[1]{\todo[inline,color=YellowOrange!60]{{\bf Giovanni:} #1}}
\newcommand{\silvio}[1]{\todo[inline,color=RoyalBlue!60]{{\bf Silvio:} #1}}
\newcommand{\vale}[1]{\todo[inline,color=Purple!60]{{\bf Valentino:} #1}}
\newcommand{\colored}[1]{\textcolor{red}{#1}}

==> AAAI 2023 SAVAGE --_ ARXIV/sections/appendice.tex <==
\section{Datasets}


\paragraph{Pruning}
Given both the high number of nodes in the social network-based datasets (Twitter and GPlus) and the high dimensionality of their feature spaces, we decided to prune them.
We started by reducing the noise in the Twitter features by normalizing the textual versions to lowercase and removing characters not allowed in the hashtag and mention as per Twitter official guidelines.\footnote{https://help.twitter.com/en/managing-your-account/twitter-username-rules\#error} Then, for Twitter, we removed features with less than 20 occurrences, and for GPlus, the ones with less than 10. After that, we pruned users with less than 20 remaining features on Twitter and 30 for GPlus. We report in Table~\ref{tab:pruning} the pruning results.



\paragraph{Preprocessing}
Considering the high-dimensionality of the majority of the dataset used and their sparsity, we adopted a preprocessing to make them smaller and, simultaneously, as denser as possible. In particular, we extracted the largest connected components from all of them. Subsequently, if the extracted subgraph had more than 10K nodes, we first sampled employing GraphSAINTSampler \cite{Zeng2020GraphSAINT}, then we retrieved the largest connected component again to ensure the density of the sampled subgraph. We report in Table~\ref{tab:dat_stat} the statistics of the preprocessed dataset.

\input{tables_supp/pruning.tex}
\input{tables_supp/dataset_stats.tex}

\section{GNN Models}

We train our link prediction system in a transductive setting, using $90\%$ of existing edges as training set and the remaining $10\%$ as test set.
We train our models for $2000$ epochs with a learning rate $lr=0.001$.
The performance of our GNN-based link prediction models measured on the test set for each dataset considered is reported in Table~\ref{tab:auc}.

\input{tables_supp/auc_table}




\section{Methods}

We have reported results for different configurations of our framework. In particular, our SAVAGE and SAVAGE-I configurations rely on a set of hyperparameters: the penalty losses $\beta$ and $\gamma$. 
In Table~\ref{tab:hyperParam} we report the best hyperparameter setting. 
These hyperparameters were found through a grid search in the range $[10^{-3}, 10]$.

\input{tables_supp/hyperParam}

\section{Ablations}

\subsection{Initialization}

As hinted several times in the paper, we are solving a highly non-convex optimization problem.
For this reason, the initialization of the perturbation matrix $P$ can be considered crucial, as it reflects both the prior information we inject into the model and the model's results itself.
For this reason, we run an ablation experiment to show how different kinds of initializations lead to different results.

We test four possible initializations for the perturbation matrix: Random, All Zeros + $\epsilon$, all Ones - $\epsilon$, and All negative ones + $\epsilon$; where $\epsilon$ is a small random positive number ($< 0.3$).
We test these options by running experiments for $20$ different pairs randomly sampled from the Synthetic dataset.

We report results in Table~\ref{tab:init_P}. We indicate the All negative ones option with a minus as footer (Ones\_).

We may observe that Random exhibits the best trade-off between the attack power and the number of resources used.

\input{tables_supp/init_P}


\subsection{Penalty losses}

SAVAGE relies on two penalty losses, $\beta$ and $\gamma$, to effectively sparsify the resources used to carry out the attack.
We hereby perform a sensitivity analysis to quantify the impact of these losses on the model results.
In particular, we sample $20$ pairs at random from the Synthetic dataset and run our method on them.

\paragraph{L-Dist}

As explained in the relevant section of the main body, $\beta$ regulates the effect of $\ldist$, that is, the penalty discouraging $\tilde{h}_{s;P}$ from being too far off from $h_s$.
In Figure~\ref{fig:abl_betas} we report our finding. On the horizontal axis, we indicate the penalty used, while on the vertical axis, the amount of resources used.
As we can see, increasing $\beta$ corresponds to a reduction in the resources used.
Furthermore, we notice that the behavior of this penalty loss is optimal, as it features a nice monotonic decrease in the amount of resources used.
While not shown here for visualization purposes, the relationships remain pretty much constant outside the range considered.

\begin{figure}[htb]
\centering
    \include{tikz/abl_betas}
    \label{fig:abl_betas}
\end{figure}

\paragraph{L-new}

As explained in the relevant section of the main body, $\gamma$ regulates the effect of $\lnew$, that is, the penalty directly discouraging the proliferation of vicious nodes injected into the original graph network.
We report results in Figure~\ref{fig:abl_gammas}.
We indicate the level of the penalty $\gamma$ used on the horizontal axis, with the amount of resources used on the vertical axis (on the log scale).
Once again, even though the intrinsic discreteness of the problem, we show how our formulation features a nice, well-behaved decrease in resources used along with the increase in the penalty loss, with an almost-monotonic curve.
While not shown here for visualization purposes, the relationships remain pretty much constant outside the range considered.

\begin{figure}[ht!]
\centering
    \include{tikz/abl_gammas}
    \label{fig:abl_gammas}
\end{figure}


\subsection{Feature Matrix}

As stated in the main body of this paper, SAVAGE does not focus on the creation of the features for the vicious nodes injected into the original graphs, focusing instead on their topology.

% \include{tables_supp/abl_X.tex}
\begin{table}[htbp]
\centering
\caption{\label{tab:X}Results under different assumptions for creating the vicious nodes feature matrix. While not optimizing for this, SAVAGE is robust under different settings and maintains strong results.}
\begin{tabular}{@{}lcccc@{}}
\toprule
Method   & AR   & AN   & AP   & KL   \\ \midrule
Existent & $0.90$  & $13.90$ & $0.90$  & $0.01$ \\
Random   & $1.00$    & $16.70$ & $0.98$ & $0.01$ \\
Ones     & $0.75$ & $42.50$ & $0.75$ & $0.01$ \\
Zeros    & $0.95$ & $14.10$ & $0.91$ & $0.01$ \\
Mean     & $0.91$ & $14.10$ & $0.91$ & $0.01$ \\
Median   & $0.95$ & $14.00$ & $0.91$ & $0.01$ \\ \bottomrule
\end{tabular}
\end{table}

In particular, we do not optimize for it, leaving it as a feature work.
However, we hereby claim that SAVAGE %as a method 
is robust under different assumptions for the creation of such a matrix.
For this experiment, once again, we sampled $20$ pairs randomly from the Synthetic dataset and ran our method on them.
This time, however, we consider six different settings for creating the feature matrix.
The first setting, used for the main experiment, is to randomly sample features from existing nodes and add a slight noise.
Three settings consist in initializing the feature matrix $X$ with zeros, ones, and at random, respectively; we apply some noise $\epsilon$ here as well.
Finally, we take the mean and the median of the feature matrix in two cases, still adding noise to it.
Results are reported in Table~\ref{tab:X}. 
These results show that we maintain strong results across different initializations.
In particular, we can notice how the Random, Zeros, and Median methods produce the strongest attack power, while Ones produces the lowest attack power while using the most resources as well.

==> AAAI 2023 SAVAGE --_ ARXIV/sections/background.tex <==
\section{Background and Notation}
\label{sec:background}
% General background and notation on graphs
We consider a {\em directed} graph $\graph$ with $n$ nodes $\V$, and $m$ edges $\edges$.
The structure of $\G$ is encoded by its adjacency matrix $\adjM \in \lbrace 0,1 \rbrace^{n \times n}$, where $\adjMij$ = 1 iff $(i, j) \in \edges$. 
Notice that, in general, $\adjMij \neq A_{j,i}$, i.e., the adjacency matrix is not symmetric.
% Nodes of $\G$ can also be associated with $k$-dimensional real vectors organized as rows of the feature matrix $\X \in \mathbb{R}^{n \times k}$.
A feature matrix $\X \in \mathbb{R}^{n \times k}$ can also be used to associate features to nodes of $\G$.
% GNN used to learn a representation of each node in G
We assume that a graph neural network (GNN) $g$ learns a hidden representation of nodes in the graph (i.e., a node embedding). Such representation is, in turn, used for our downstream task of interest (i.e., link prediction).

% Node's neighbors and neighborhood
The embedding of each node is learned through $g$ by iteratively updating the node's features based on the neighbors' features.
Formally, let $\h^l_u$ denote the embedding of node $u\in \V$ at the $l$-th layer of $g$. 

Let $\neigh^1(u) = \neigh(u) = \{v\in \V~|~(u,v)\in \edges\}$ be the $1$-hop neighborhood of $u\in \V$, i.e., the set of all nodes that are adjacent to $u$.
More generally, we can define the $l$-hop neighborhood of $u$ ($l\in \Z^+,~l > 1$) as the set of nodes that are {\em at most} $l$ hops away from $u$, using the following recurrence relation:
\[
\neigh^l(u) = \neigh^1(u) \cup \bigcup_{v\in \neigh(u)} \neigh^{l-1}(v).
\]
Hence, let us consider the subgraph $\G^l_u$ of $\G$ induced by $u$ and its $l$-hop neighborhood $\neigh^l(u)$ as relevant for the computation of $\h^l_u$. 
Specifically, we consider $\adjM^l_u$ and $\X^l_u$ as the adjacency matrix and the feature matrix of nodes in the subgraph $\G^l_u$, respectively, and $\h^l_u$ is computed by $g$ using the following equation:
\begin{equation}
    \label{eq:gnn-emb}
    \h^l_u = g(\adjM^l_u,\X^l_u;\params_g) = \phi(\h^{l-1}_u, \psi(\{\h^{l-1}_v~|~v\in \neigh(u)\})),
\end{equation}
where $\phi$ and $\psi$ are arbitrary differentiable functions (i.e., neural networks): $\psi$ is a permutation-invariant operator that {\em aggregates} the information from the $l$-hop neighborhood of $u$; $\phi$ {\em updates} the node embedding of $u$ by combining information from the previous layer; $\params_g$ are the trainable parameters of $g$.
The number of hidden layers in $g$ determines the set of neighbors included while learning each node's embedding.
From now on, unless otherwise needed, we will consider $l$ fixed and omit the corresponding superscript.

% The link prediction problem
% Given the graph $\Gobs=(\V, \edgesobs)$, where $\edgesobs \subset \edges$ is a subset of the true links observed, the {\em link prediction} problem can be formulated as a binary classification task, whose goal is to learn a function $f: \V \times \V \mapsto \labels$, where $\labels = \{0,1\}$\footnote{Same considerations apply when $\labels = \{-1,1\}$.}, that indicates if there exists an edge between any two nodes. 
% More formally, $f(u,v) = 1$ iff $(u,v)\in \edges\setminus \edgesobs$. 
% In the probabilistic formulation, instead, the link prediction resorts to estimating the probability that an edge exists between two nodes, i.e., $f(u,v) = \Prob[(u,v)\in \edges \setminus \edgesobs]$.
Given the graph $\Gobs=(\V, \edgesobs)$, where $\edgesobs \subset \edges$ is a subset of the true links observed, the {\em link prediction} problem generally resorts to estimating the probability that an edge exists between two nodes $u$ and $v$, i.e., $\Prob[(u,v)\in \edges \setminus \edgesobs]$.
%\fabri{We should say how we compute $\Prob$.}
%\gabri{Tipo?}
%\fabri{Ho fatto questo commento prima di leggere dopo. Forse siamo stati un po' troppo lunghi. Forse basta dire che P e' calcolata come f che e' una rete neurale. Senza stare a dire che c'e' una f pero' noi non la conosciamo, ecc. ecc. Quello e' sempre lo stesso problema di non conoscere la distro, no?}

% Link prediction using GNN
Let $\h_w = g(\adjM_w,\X_w;\params_g)$ be the embedding of the generic node $w\in \V$.
Thus, we assume that the predicted link probability between two nodes $u$ and $v$ is approximated with a function $f$, defined as follows:
\begin{equation}
\label{eq:gnn-lp}
    f(\h_u, \h_v; \params_f) = f (g(\adjM_u,\X_u;\params_g), g(\adjM_v,\X_v;\params_g); \params_f).
\end{equation}

Notice that $f$ can itself be another neural network (e.g., an MLP) that takes as input two node embeddings learned by the GNN $g$ and outputs their link prediction. 


%\fabri{$g$ viene definita come dipendente da $\w$ e poi questo scompare. Inoltre, non e' chiaro che rapporto c'e' tra $\params$ e $\w$? Forse dovremmo tenerli separati? Forse chiamarli $\params_g$ e $\params_w$?}
%\gabri{Vero, scompaiono i parametri per alleggerire un po' la notazione... però lo diciamo sopra cosa si intente per $\params$. In particolare: The overall set of end-to-end trainable parameters is denoted by $\params$ and includes also the parameters $\w$ of $g$. Mi piace anche quello che proponi tu, però non so se appesantiamo davvero tanto la notazione (per correttezza penso che sia $\params_g$ e $\params_{f}$...}

% A combined embedding $\h_{u,v}$ of the two input nodes can be simply obtained via dot product ($\h_{u,v} = \h_u^T \cdot \h_v$) or element-wise product ($\h_{u,v} = \h_u \odot \h_v$).
A combined embedding $\h_{u,v}$ of the two input nodes can be obtained, for example, via Hadamard (element-wise) product, i.e., $\h_{u,v} = \h_u \odot \h_v$.
%\fabri{Il dot product ritorna un numero, ci va bene come embedding?}
%\gabri{True... questa cosa mi pare di averla presa in prestito da un altro paper ma in effetti hai ragione...}
Eventually, the probability of a link existing between $u$ and $v$ can be computed as $f(\h_u, \h_v;\params_f) = \sigma(\params_f^T\h_{u,v})$, where  $\sigma(x) = \frac{1}{1+e^{-x}}$ is the sigmoid activation function at the last output layer of $f$.

In the following, we denote as $\params$ the overall set of end-to-end trainable parameters of $f$ and $g$, i.e., $\params = \left[\params_f, \params_g\right]$.


==> AAAI 2023 SAVAGE --_ ARXIV/sections/conclusion.tex <==
\section{Conclusion and Future Work}
\label{sec:conclusion}
%\gio{Qui quindi ci vogliamo mettere come limitazione che aggiungiamo tanti archi? Secondo me dobbiamo stare attenti, perche' stressiamo il fatto che usiamo poche risorse, e poi diciamo che ne usiamo tante... forse ora che usiamo la KL ce la possiamo cavare cosi?}
In this work, we presented \savag, a novel framework for generating adversarial attacks on GNN-based link prediction systems.
\savag\ defines a white-box attack model where an adversary aims to appear in the list of recommended users to follow for a target victim node.
The attacker controls a subset of original nodes and some additional vicious nodes that can inject into the network. Each of these malicious nodes can, in turn, create or destroy direct edges with others until eventually altering the link prediction between the target victim node and the attacker node.
\savag\ formulated the problem that the attacker must solve as an optimization task, which trades off between the attack's success and the sparsity of malicious resources required.
Experiments conducted on real-world and synthetic datasets showed the effectiveness and efficiency of our approach in attacking several GNN-based link prediction models. Moreover, we showed that \savag\ attacks can be successfully transferred to disrupt other link prediction systems (not necessarily GNN-based) under black-box setting.
In future work, we plan to extend our attack model with the ability to perturb node features. 
Furthermore, our method must operate on dense adjacency matrices, somewhat limiting its scalability. 
Thus, we will develop a variant of \savag\ that can work with sparse adjacency matrices.
The design of possible defense mechanisms to combat the attacks generated by \savag\ is another interesting direction to explore; we will also consider different downstream tasks as the target of the attacks (e.g., node classification).
%\vale{E se mettessimo nei future work l'attaccare altri tipi di task? Cosi' preveniamo commenti tipo "ma perche' non attaccate node classification?!" rispondendo subito}
% Finally, inspired by social networks, we focused on directed graphs; however, an extension to undirected graphs would be worth of being explored.



==> AAAI 2023 SAVAGE --_ ARXIV/sections/experiments.tex <==
\section{Experiments}
\label{sec:experiments}

We evaluate the effectiveness of \savag\ on several challenges.
First, we assess the power of our attack model by reporting some key performance metrics.
Second, we analyze the impact of the critical components of our model through ablation studies.
Finally, we demonstrate the ability of \savag\ to generate attacks that transfer toward other black-box link prediction systems.
We have released code on Github \footnote{https://github.com/GiovanniTRA/SAVAGE}.

\subsection{Experimental Setting}

\paragraph{Datasets.}
We validate our method both on real-world and synthetic datasets.
Moreover, as dictated by our attack model, we focus only on data representing {\em directed} graphs. 
Our real world datasets are mainly of two kinds: citation-based and social networks.
The former category includes \emph{Cora}~\cite{kunegis2013konect, vsubelj2013model}, \emph{Arxiv}~\cite{wang2020microsoft}, and \emph{Citation2}~\cite{wang2020microsoft}, whereas the latter contains \emph{Twitter}~\cite{leskovec2012learning}, \emph{Wikipedia-Vote}~\cite{leskovec2010signed, leskovec2010predicting}, and \emph{GPlus}~\cite{leskovec2012learning}.
Furthermore, we test our method on a synthetic dataset, partially taken from~\cite{Fey2019FastGR}, that we call \emph{Synthetic}.
It is worth noticing that, to properly test our method, we choose datasets featuring a varying degree of cardinality and density.
For further details on the preprocessing steps taken and additional statistics, we refer the reader to the supplementary material.


\paragraph{GNN Models.}
To evaluate the effectiveness of \savag, we first train a GNN-based link prediction system. The model is composed of two stacked convolutional layers of 128 and 64 hidden units, respectively, and a two-layer MLP with a sigmoid activation function at the last output layer.
In our setup, we minimize the prediction error with a binary cross-entropy loss using Adam optimizer with $3\times 10^{-3}$ learning rate. 
Finally, we compute the accuracy (using $0.6$ as classification threshold) and the AUROC (Area Under the ROC) curve of the learned GNN-based link predictor.  
On average, the best model achieves $85\%$ accuracy and $0.86$ AUROC score on every dataset considered. 
The full details are available in the supplementary material.


\paragraph{Methods.}
We test our method against different competitors and under several settings.
First, we consider a simple random baseline (RAND). 
This can add/remove connections in the graph and activate/deactivate vicious nodes with a probability $p$; the larger $p$, the stronger the corresponding attacker. 
We denote by RAND-L and RAND-H the baseline with the lowest and the highest probability of addition/activation, i.e., $p_\text{L} = 0.25$ and $p_\text{H} = 0.75$.
While we cannot perform a direct comparison with other methods, as they are not naturally designed for our setting, we adapt the greedy technique proposed in~\cite{wang2018attack} and~\cite{chen2020link} to work in our framework, and we call it AIGA (Adapted Iterative Gradient Attack). 
Finally, we consider four instances of our method: {\em(i)} \savag, {\em(ii)} \savag-N,  {\em(iii)} \savag-I, and  {\em(iv)} \savag-NI. 
\savag\ refers to the plain full framework, randomly initialized and defined in Eq.~\ref{eq:instance-loss}; \savag-N is the same as \savag\ yet without the penalty losses (i.e., $\ldist$ and $\lnew$); \savag-I is the same as \savag\ yet initialized with the output from AIGA; and \savag-NI is the same as \savag-N yet initialized with the output from AIGA.
Since \savag\ tries to solve a highly non-convex problem, the initialization of the parameters is indeed crucial. Distinguishing between random and AIGA-based initialization serves two purposes.
First, it shows that \savag\ can be used just as a sparsifying framework, compatible with other techniques; second, it demonstrates the impact of initialization on the optimization problem.
For all the models considered, performance is reported according to their best hyperparameter setting, which is detailed in the supplementary material.


\paragraph{Evaluation Metrics.}
Given a graph and a GNN-based link prediction model trained on it, we uniformly sample a source and a target node from the graph, providing that the two nodes are disconnected and, even further, they are not part of each other's 2-hop neighborhood. Moreover, according to the link prediction model, no edge should exist between the two sampled nodes. 
Then, we attack the graph using all the methods described above (i.e., the four variants of our \savag\ along with its competitors) and run again the link prediction on the resulting perturbed graph.
We repeat this procedure for 20 different node pairs, for each dataset used.
We present our results according to the following metrics.
The average prediction under attack (AP) is the estimated probability output by the link prediction model {\em after} the attack.
The attack rate (AR) measures the fraction of successful attacks, i.e., it counts the fraction of predictions above the success threshold ($0.6$). %\footnote{We report both AP and AR as the latter may saturate.}
% It is worth noticing that 
AP and AR capture two different aspects of the attack power. The former indicates the average {\em strength} of each attack (i.e., the new link probability between the source and target node, which initially was below the success threshold). The latter measures only how frequently the new link probability is large enough for the attack to succeed, regardless of its actual value.
Finally, we report statistics on the perturbation induced by \savag\ on the original graph topology: the number of vicious nodes injected (AN) and the shift in the node's degree distribution {\em before} and {\em after} the attack as measured with the Kullback-Leibler divergence (KL).




% and the number of perturbed edges (AE).

\subsection{Attack Power}
We measure the power of the attacks generated by all the methods examined on the real-world and synthetic datasets; the results are shown in Table~\ref{tab:vn_result}.
We may observe that \savag\ can mount very effective attacks across all datasets, with the highest AP and AR between all the considered methods. 
In terms of AR, we notice a positive correlation between the performance gap and the density of the dataset.
Furthermore, \savag\ significantly reduces the number of malicious resources used (AN) w.r.t. to AIGA, ranging from a minimum of 20\% up to 80\% decrease and the KL score illustrates the limited impact on graph connectivity, especially when compared with the baselines (see Section~\ref{subsec:limit} for additional discussion). 
We observe that the AIGA initialization can further mitigate this impact at the cost of a slightly worse AR in sparser graphs. This may be caused by the initialization that imposes the solution to get stuck around the starting local minimum.
In other words, this analysis shows that \savag\: {\em (i)} generates more successful attacks than competitors, {\em (ii)} with stronger confidence, and {\em(iii)} does not rely on the introduction of random noise since random baselines are not able to disrupt the prediction even when using a comparable number of resources.

% \input{tables/s_svn_table}
\input{tables/vn_table}

% \paragraph{Enforcing Sparsity.}
% \input{tables/ablation_X}
\subsection{Ablation Study}

We perform an extensive ablation study to support the design choices made for the main components of our framework.
A key characteristic of \savag\ is its ability to enforce sparsity of malicious resources by adjusting the optimization goal of the attacker.
We analyze several components of the model, like the initialization of the perturbation matrix and the effect of the penalty losses, to study their behavior and how this impacts the sparsification effort.

\begin{figure}
    \centering
    \includegraphics[scale=0.16]{images/visual_aaai23.png}
    \caption{Visualizations of gradients for the model with $\ldist$ and $\lnew$ (left), and without (right). Each cell describes the activation strength of a vicious node. In blue are deactivated nodes. We (visually) show that our losses successfully induce a sparse usage of malicious resources.}
    \label{fig:sparse_matrix}
\end{figure}

We provide here a graphic visualization of our findings on \savag\ inner working.
In Fig.~\ref{fig:sparse_matrix}, we inspect the gradients of our model with our introduced sparsity losses $\ldist$ and $\lnew$ (left) against the model not featuring them (right).
It is highly evident that most vicious nodes on the left are deactivated (encoded with blue), and do not contribute as additional resources to mount the attack.
This is not true for gradients on the right, which instead have a much higher diffusion, with credits being awarded to the largest number of vicious nodes possible.
Thus, we argue this is further proof that our formulation is effective in injecting sparsity into the model, making more efficient usage of malicious resources.
Again, we remind that we do not directly optimize for the feature matrix of the graph, focusing instead on its topology, and leaving it for future work.
Still, we conduct a comprehensive analysis, showing that \savag\ is robust under different assumptions for the creation of the vicious nodes' features.
For the entire set of results from our ablation study we refer the reader to the supplementary material.










% Unlike existing approaches, our method is able to enforce sparsity of malicious resources by adjusting the optimization goal of the attacker. 
% In~\ref{fig:teaser}, we can inspect the gradients of our model with our special sparsity losses against the model that does not feature them.



% \begin{figure}[]
% \begin{center}
% \includegraphics[width=0.7\columnwidth]{images/visual_nips_22.png}
% \end{center}
% \caption{\label{fig:grad} 
% Visualizations of gradients for the model with our losses (left), and without (right). Each cell describes the activation strength of a vicious nodes. In blue are deactivated nodes. Again, we (visually) show that our losses successfully introduced sparsity in the resources used.}
% \end{figure}


\subsection{Attack Transferability}
\label{subsec:transf}

%Our threat model can be considered as a white-box attack. However, we claim that the adversarial perturbation generated with our method is transferable to fool other methods for link prediction initially unaccounted for.
\savag\ defines a white-box attack model, i.e., it assumes a full knowledge of the target GNN-based link prediction model. 
This assumption may be unrealistic in practice; indeed, the internals of a link prediction system (e.g., the model's architecture, parameters, or gradients) are rarely disclosed, especially in a commercial scenario.
Nevertheless, we claim that this restriction does not limit the feasibility of our method. 
In fact, we show that the adversarial perturbations generated by \savag\ can be successfully transferred to fool other link prediction systems (not necessarily GNN-based) under the more challenging black-box setting.
Specifically, to demonstrate this capability, we focus on several link prediction heuristics, as reported in Table~\ref{tab:tra_alg}.
The higher the value of these heuristics, the higher the chance of a link between two nodes. 
%The table summarizes the heuristics scores and their definition. 
For a given graph, a source and a target node initially disconnected, and a white-box GNN-based link predictor, we generate the corresponding perturbation with \savag\ so to increase the probability of a connection between the victim and the source. 
%Then, we compute each heuristic value considered, before and after the graph perturbation occurs.
The scores in Table~\ref{tab:tra_alg} are expressed in terms of the lift of the heuristic values as computed in the original, unperturbed graph, i.e., before and after the attack, averaged across 20 different pairs of sampled source and target nodes.
We observe an increase of all the heuristic values considered, which indicates that \savag\ would be able to mount attacks even on non-GNN-based link prediction systems.
% Specifically, to demonstrate this capability, we focus on the following link prediction heuristics for directed graphs: Katz Index~\cite{katz1953new}, personalized PageRank~\cite{BRIN1998107} and SimRank~\cite{10.1145/775047.775126}.
% Table~\ref{tab:tra_alg} summarizes the heuristics and their definition, along with the improvement we obtain over the initial, unperturbed, condition.
% Notice that, given our way of sampling node pairs, the original score obtained with these heuristics is either $0$ or alike. The improvement is expressed then as the differential normalized by the number of nodes in the graph.
% \gabri{We need to stress much better this part on the attack transferability!}
% \gio{Abbiamo raddoppiato il numero di metriche... secondo te cosa possiamo fare in piu?}

\input{tables/transferability_alg}

\subsection{Limitations}
\label{subsec:limit}
Experiments have demonstrated that \savag\ can achieve a high attack success rate while using a sparse number of new, malicious nodes.
However, \savag\ causes a shift in the node's degree distribution between the original and the attacked graph larger than other methods, thus indicating a more substantial perturbation of the initial graph links.
We argue that, in general, from the attacker's perspective, the cost of adding a vicious node to the network is the most relevant and that should receive the highest priority.
Moreover, on average, the KL-divergence between the two node distributions is smaller than $10^{-3}$ with \savag. Still, we acknowledge this as a limitation of our current method.
We plan to incorporate a new factor (based on the KL-divergence above) in the attacker's objective, limiting the impact of \savag\ on the original graph connections. 

% \vale{Non potrebbero dirci subito "ok, ma perche' non lo avete gia' fatto se lo sapete ed e' qualcosa che gia' usate per misurare proprio le prestazioni?". Lo stiamo dicendo qui perche' siamo consci del fatto che l'avremmo dovuto fare e quindi preveniamo la critica? Proporrei qualcosa come "..of our current method and we plan to work on a constraint to account for the quantity of the new edges added"}
% \gabri{L'ho riscritta come sopra... cosa ne pensate?}












% In this section, we justify our choices on hyperparameters, and we present some insights into the key properties of our method with an in-depth analysis.

% \paragraph{Transformations.}
% We report results for different transformations of the perturbation parameters on the \emph{obgn-arxiv} dataset in a simplified setting (fewer optimization steps and vicious nodes controlled) to appreciate the differences between the maps better.
% As stated earlier, we solve an inherently discrete optimization problem by learning a set of continuous transformations of the perturbation parameters.
% The choice of these transformations is crucial to close the gap between the optimal continuous solution and the discrete one required by our problem. 
% In this experiment, we try different potential setups; results are shown in Table~\ref{tab:abl_tr}.
% \input{tables/ablation_transform}
% We observe that the set of crafted transformations are very effective and vastly improve results over the baseline (\emph{none}). Intuitively, by using the $\tanh$ function, we guide the optimization toward values that are closer to discrete operations (i.e., adding/remove edges). It is worth noticing that the results are worst when using the $\clamp$ function exclusively. This is because those values outside its range do not get a gradient, making the optimization impossible.
% On the other hand, when applying a $\tanh$ on the perturbation parameters $P$ and a $\clamp$ to activate/deactivate nodes, results are on par with the previous option.
% Finally, by removing the $\clamp$ on $\advadjM_s$ results collapse. \gabri{Cosa vogliamo dire sopra? Inoltre, ha senso presentare un risultato in cui non facciamo clamp sulla matrice $\advadjM_s$?}
% While we find the optimal solution to the continuous problem (the output of the GNN model is $1$), we loose the possibility of optimizing our original problem.

% \paragraph{Initialization of Vicious Nodes Features}

% While our method does not optimize for the best nodes feature representation, we are still influenced it.
% For this reason we analyze the impact of different possible initialization for the feature matrix of the vicious nodes created....


















% For real-world datasets, we rely on OpenGraphBenchmark~\cite{hu2020ogb}, a collection of freely-available large scale graphs. 
% In particular, we use two datasets from this repository: \textit{obgn-arxiv}~\cite{wang2020microsoft} and \textit{ogbl-citation2}~\cite{wang2020microsoft}.
% They both refer to directed graphs representing two different citation networks: the former contains all computer science (CS) arXiv papers, whereas the latter contains a subset of papers extracted from MAG~\cite{paetzold2021graphdata}.
% Each node represents a paper with 128-dimensional word2vec~\cite{NIPS2013_9aa42b31} features that summarize its title and abstract, and a directed edge indicates that one paper cites another.

%The first one is \textit{obgn-arXiv}~\cite{wang2020microsoft}, which is a directed graph representing the citation network between all Computer Science (CS) arXiv papers. Each node represents an arXiv article, each directed edge indicates that a paper references another one. The second dataset used is \textit{ogbl-citation2}~\cite{wang2020microsoft}. This is a directed graph that represents the citation network between a selection of articles. Each node represents a paper with 128-dimensional word2vec~\cite{NIPS2013_9aa42b31} features that summarize its title and abstract, and each directed edge shows that one paper cites another.
% For both datasets, we sample the subgraph with the largest connected components. 
% As a result, we obtain a graph with 10,697 nodes and 46,624 edges for {\em obgn-arxiv}, and one with 10,124 nodes and 15,359 edges for {\em ogbl-citation2}.

% Since a few datasets of directed graphs with node features are publicly available, we test our model also on a synthetic dataset. For this purpose, we rely on PyG~\cite{Fey2019FastGR} class for random datasets.
% Specifically, we create a synthetic, directed graph with 3,192 nodes with 64 features each and 31,857 edges.
% However, in this setting, edges are created randomly between nodes; therefore, a link prediction model can't learn anything but noise. Still, we show that \savag\ can attack even such systems.
% In our synthetic configuration, we have randomly created a directed graph with $3,192$ nodes with $64$ features each and $31,857$ edges.


%Finally, we gladly notice that not only our attack rates are high but, even more importantly, the confidence measured in link probability (AP) is convincing.
% As stated earlier, we consider several attack scenarios; namely, an attacker may control itself ({\em source}), only a set of vicious nodes ({\em vicious}), or both ({\em source} + {\em vicious}).
% For all of these scenarios, we report on the metrics defined above.
% Furthermore, we show the difference between the case without the penalty losses and the one which instead includes it (identified with an extra ``$(L)$'').







% In Table~\ref{tab:s_svn_result}, we can see that when the attacker controls the source node only is very effective. However the amount of perturbed edges is massive. This is accounted for by introducing our loss, resulting in attack that uses a fraction of the resources ($\beta = 10$ is the penalty used).

% In Table~\ref{tab:vn_result}, we show the results for the remaining settings.
% Again, we observe that the plain attack, although very effective, is very eager of malicious resources.
% \gio{Come gestiamo tutti i beta vari che abbiamo usato? secondo me potremmo anche non parlarne, tanto abbiamo gli ablation appositi.}
% On the other hand, our model efficiently introduces sparsity with competing results: $\beta=0.1 / 0.01$ and $\gamma=3e-2 / 15e-3$ for the {\em source} + {\em vicious} and {\em vicious} setup, respectively.




% In particular, we explore different scenarios compliant with our attack model and mounted using our framework.
% We call {\em source} the setup in which the attacker is able to control only itself. We then explore a case where the attacker cannot only control its actions but also create vicious nodes and control them ({\em source} + {\em vicious}). Finally, we consider the possibility that the attacker might not want to take action personally but delegates off the task of attacking a target exclusively to the vicious nodes ({\em vicious}).




==> AAAI 2023 SAVAGE --_ ARXIV/sections/introduction.tex <==
\section{Introduction}
\label{sec:intro}


\blfootnote{$\dagger$ Equal Contribution}
% The explosive growth of digital social media platforms in the last two decades has produced networks containing millions or even billions of users.
% Different from real-life social networks, where bonds amongst people arise naturally from the human beings involved, the scale of digital social networks has opened up the opportunity for automatic (i.e., machine-based) systems that can suggest the creation of new connections between people.
% This is precisely the purpose of \emph{link prediction} methods.
%The purpose of {\em link prediction} methods is to automatically suggest the creation of new connections between social network users. 
%Informally, these methods estimate the probability that a link between two users should exist~\cite{martinez2016survey,kumar2020link}.
The purpose of {\em link prediction} methods is to estimate the probability that an edge between two initially disconnected nodes in a graph should exist~\cite{martinez2016cs,kumar2020link}. 
For example, these methods are used to suggest the creation of new connections between social network users (e.g., follower-followee relationships).

Several approaches to link prediction have been proposed in the literature~\cite{lu2011link}. 
Recently, methods based on graph neural networks (GNNs) have achieved state-of-the-art performance~\cite{kipf2016semi}.

The list of predicted links for a given user ranked by their estimated probability represents a set of recommended new contacts, which eventually the user may decide to follow or not.
This step is crucial, especially for some authoritative, highly followed social network users, i.e., so-called ``{\em influencers}''.
Indeed, their reputation (and therefore social market value) may be affected by who they choose to follow.
Specifically, when the target of recommendations is an influencer, it is paramount to be accurate at suggesting the ``right'' set of candidate users to follow. 
As a matter of fact, being followed by an authoritative user can be seen as a sign of endorsement and ultimately could bring several advantages to the followee (e.g., higher revenue from advertising campaigns run on the social media platform due to increased popularity).
Hence, malicious users have a strong interest in {\em manipulating} link recommendation systems to inflate their reputation on social media platforms artificially, thus perpetuating their own (harmful) goals through adversarial attacks.
For example, consider Sammy is a social network user interested in increasing their reputation.
Ideally, they would have other influential users follow them to reach this goal..
However, Sammy has no control over other users, 
making such tactic unfeasible.
Still, Sammy could try to adjust their existing connections (i.e., follow/unfollow users) with the hope that their name will show up in the list of recommended connections for Terry, i.e., the user profile of a target influencer.
More generally, Sammy would control a subset of nodes (in addition to themselves) and is allowed to modify their neighborhood to achieve their goal. 
Sammy may also be able to inject {\em new} nodes in the network and create connections between such ``artificial'' users and other existing nodes.
Obviously, all these operations (e.g., adding/deleting an edge between two nodes) have a cost, which Sammy wants to account for and minimize. 
Although the body of work on adversarial attacks on link prediction is extensive~\cite{sun2018adversarial}, most of the literature do not completely cover the scenario described in the example above. 
Indeed, most work assumes the attacker can perturb the original network topology by adding or deleting connections only between {\em existing} nodes to favor the malicious goal~\cite{chen2020link}.
However, this setting is often unfeasible because it requires the direct control of real users, with prohibitive coordination costs.
To overcome this limitation, vicious node adversarial attacks have been proposed~\cite{wang2018attack}.
Under this setting, the attacker can create new users {\em ex-novo} and, by controlling these nodes, engineer the network to mount the attack.
This approach is much more feasible than directly controlling real nodes; indeed, the Internet is full of services selling fake accounts/comments/likes.

%Recently, Elon Musk's offer to acquire Twitter has been withdrawn, allegedly, due to the large number of fake users (bots) found, with the entrepreneur claiming that around 10\% of its monetizable daily active users fall into this category~\cite{musk5}.

Still, existing methods for implementing vicious node attacks do not incorporate the cost of adding such malicious nodes into the adversary's objective~\cite{wang2018attack}. 
Those methods typically assume the existence of an upper bound on the attacker's budget allocation, which is generally exhausted to favor the highest attack success rate possible.
In other words, if an attacker has a maximum allowed budget of $N$ vicious nodes to inject into the network, it will use all of them to increase the chance of attack success.
We argue that this solution is inefficient and impractical.
%\fabri{Io definirei esplicitamente il termine vicious attack. Non si capisce cosa si intende, secondo me}
For this reason, in this paper we introduce \savag\ ({\em \textbf{S}p\textbf{A}rse \textbf{V}icious \textbf{A}ttacks on \textbf{G}raph n\textbf{E}tworks}).
This is a novel framework that provides an original perspective on vicious node adversarial attacks on GNN-based link prediction methods for {\em directed} graphs. 
\savag\ operates in a white-box setting and promotes a spare use of the malicious resources required by the attacker, i.e., the number of vicious nodes and their aggressiveness.
Moreover, \savag\ is general enough as it allows to frame existing vicious node attacks into it. 
%In this context, we propose \savag\ ({\em \textbf{S}p\textbf{A}rse \textbf{V}icious \textbf{A}ttacks on \textbf{G}raph n\textbf{E}tworks}), a novel method that is coherent with the framework just introduced.
%\gabri{Se introduciamo il nome del metodo all'inizio del paragrafo (come ho fatto adesso), la frase sopra secondo me si può tranquillamente togliere... In altre parole, vogliamo mantenere anche qui la distinzione tra framework e metodo?}

% \begin{figure}[]
% \begin{center}
% \includegraphics[width=\textwidth]{images/teaser_nips22_prova.png}
% \end{center}
% \caption{\label{fig:teaser} 
% The image shows a sample direct graph. Yellow nodes are the source of the attack, while blue nodes are the target. Red nodes are the injected vicious nodes. Previous methods aim to maximize the strength of the attack (middle), maybe under some upper bound constraint. On the other hand, \savag\ (right) enforce sparsity on the amount of resources used, while maintaining strong results.}
% \end{figure}

% \begin{figure}
%     \centering
%     \includegraphics[scale=0.25]{images/SAVAGE.png}
%     \caption{Caption}
%     \label{fig:my_label}
% \end{figure}

% \begin{figure*}
%     \centering
%     \includesvg[scale=0.5]{images/SAVAGE.svg}
%     \caption{\silvio{Che ne pensate se gli aggiungiamo (a), (b), (c) alle sottofigure? Inoltre potremmo aggiungere S (source) e T (target) all'interno dei nodi.} 
%     \gabri{Sì, provo a rifarla io questa figura: pensavo proprio di aggiungere $s$ e $t$ e (a), (b) e (c)}
%     The image shows a simple direct graph. Yellow nodes are the source of the attack, while blue nodes are the target, with green representing other nodes in the graph. Red nodes are the injected vicious nodes. Previous methods saturate the allocated budget (middle). On the other hand, \savag\ (right) enforce sparsity on the amount of resources used, deactivating resources (grayed-out nodes), while maintaining strong results.}
%     \label{fig:teaser}
% \end{figure*}

\begin{figure*}
    \centering
    \begin{subfigure}[h]{0.3\textwidth}
        \includegraphics[width=\textwidth]{images/original-graph}
        \caption{The original {\em directed} graph.}
        \label{fig:graph-ori}
    \end{subfigure}
    ~ %add desired spacing between images, e. g. ~, \quad, \qquad, \hfill etc. 
      %(or a blank line to force the subfigure onto a new line)
    \begin{subfigure}[h]{0.3\textwidth}
        \includegraphics[width=\textwidth]{images/perturbed-graph}
        \caption{A generic attack to mispredict the existence of the link between $t$ and $s$.}
        \label{fig:graph-perturbed}
    \end{subfigure}
    ~ %add desired spacing between images, e. g. ~, \quad, \qquad, \hfill etc. 
    %(or a blank line to force the subfigure onto a new line)
    \begin{subfigure}[h]{0.3\textwidth}
        \includegraphics[width=\textwidth]{images/perturbed-graph-savage}
        \caption{The attack generated by \savag\ is still successful but uses a sparser number of malicious resources.}
        \label{fig:graph-perturbed-savage}
    \end{subfigure}
    \caption{The picture on the left (a) shows a simple directed graph, where the red node indicates the {\em source} ($s$) and the blue node the {\em target} ($t$) of the link prediction attack. In the middle (b), a generic attack is depicted: the injection of vicious nodes (in purple) and new connections induce the link prediction system to suggest the connection between $t$ and $s$. Typically, these attacks exhaust the allocated attacker's budget. On the other hand, \savag\ (c) enforces sparsity on the amount of malicious resources used, deactivating unnecessary vicious nodes (grayed-out), while keeping the attack successful.}\label{fig:teaser}
\end{figure*}





% \begin{figure}
    
%     \includegraphics[scale=0.45]{images/teaser_nips22_prova_2.png}
%     \hspace{0.5 cm}
%     \includegraphics[scale=0.13]{images/visual_nips_22.png}
%     \caption{\textbf{(left)} The image shows a sample direct graph. Yellow nodes are the source of the attack, while blue nodes are the target. Red nodes are the injected vicious nodes. Previous methods aim to maximize the strength of the attack (middle), maybe under some upper bound constraint. On the other hand, \savag\ (right) enforce sparsity on the amount of resources used, while maintaining strong results. 
%     \textbf{(right)} Visualizations of gradients for the model with our losses (left), and without (right). Each cell describes the activation strength of a vicious nodes. In blue are deactivated nodes. Again, we (visually) show that our losses successfully introduced sparsity in the resources used.}
%     \label{fig:teaser}
% \end{figure}





%In the present paper, we are proposing the following innovative contributions:
Overall, the main novel contributions of this paper are as follows:
\textbf{(a)} We introduce \savag, a novel framework that enables a comprehensive attack model based on vicious nodes to generate adversarial attacks on GNN-based link prediction systems;
\textbf{(b)} \savag\ trades off the power of the attack with the number of malicious resources required by explicitly enforcing the sparsity of vicious controlled nodes without assuming any constraint on the attacker's budget;
\textbf{(c)} We show the feasibility and effectiveness of \savag\ in attacking several GNN-based link prediction models learned from real-world and synthetic datasets through extensive experiments;
\textbf{(d)} We demonstrate that adversarial attacks generated with \savag\ can be successfully transferred to harm other link prediction systems (not necessarily GNN-based) under the more challenging black-box setting.

All code and data is released as supplementary material. 



% \begin{itemize}
%     % NEW FRAMEWORK & METHOD
%     \item We introduce \savag, a novel framework and a method that enables a comprehensive attack model based on vicious nodes to generate adversarial attacks on GNN-based link prediction systems.
%     % SPARSE VICIOUS ATTACK
%     \item \savag\ trades off the power of the attack with the number of malicious resources required by explicitly enforcing the sparsity of vicious controlled nodes without assuming any constraint on the attacker's budget.
%     % FEASIBILITY/EFFECTIVENESS OF THE ATTACK (ATTACK SUCCESS RATE?)
%     \item We show the feasibility and effectiveness of \savag\ in attacking several GNN-based link prediction models learned from real-world and synthetic datasets through extensive experiments.
%     % TRANSFERABILITY
%     \item We demonstrate that adversarial attacks generated with \savag\ can be successfully transferred to harm other link prediction systems (not necessarily GNN-based) under the more challenging black-box setting.
% \end{itemize}
%\gabri{Da rivedere la lista dei contributi sopra...}





==> AAAI 2023 SAVAGE --_ ARXIV/sections/method.tex <==
\section{Method}
\label{sec:method}
In this section, we describe the method used by the attacker to solve the optimization problem defined in Eq.~\ref{eq:optimal-emb}, which we overall refer to as \savag.

We consider the function $\pi$ parametrized by a perturbation matrix $P$, i.e., $\pi(\cdot;P)$, and thus rewrite Eq.~\ref{eq:pi} as follows:
\begin{equation}
\label{eq:pi_v2}
    \advh_{s;P} = g(\pi(\adjM'; P), X_s) = g((P\oplus \adjM'), X_s) = g(\advadjM_s, \X_s),
\end{equation}
% \begin{equation}
% \label{eq:pi_v2}
%     \advh_{s;P} = \pi(\h_s; P) = g(\pi(\adjM'; P), X_s) = g((P\oplus \adjM'), X_s) = g(\advadjM_s, \X_s),
% \end{equation}
namely $\advadjM_s = \pi(\adjM'; P) = P\oplus \adjM'$, where $\oplus$ is the element-wise matrix addition.

The perturbation matrix $P\in \{-1,0,1\}^{n\times n}$ is a discrete squared matrix, where $n = |\V'|$ is the total number of nodes of the augmented graph $\G' = (\V',\edges)$. 
This includes the set of additional vicious nodes $\Vnew$ injected by the attacker into the original graph $\graph$ (i.e., $\V' = \V\cup \Vnew$), yet keeping the same set of original edges $\edges$, thus is represented by the adjacency matrix $\adjM'$. 
For each $i\in \V^s \cup \Vnew, j \in \V'$:
\[
  P_{i,j} =
  \begin{cases}
    +1 & \text{if $(i,j)\in \edges^+$: {\em add} the edge between $i$ and $j$,}\\% and $j\in \V'$,}\\
    -1 & \text{if $(i,j)\in \edges^-$: {\em remove} the edge between $i$ and $j$,}\\% $i\in \V^s \cup \Vnew$ and $j\in \V'$,}\\
    0 & \text{otherwise.}
  \end{cases}
\]
Hence, for a given perturbation matrix $P$, a graph $\G'$ with $\Vnew$ vicious nodes, a pair of source (attacker) and target (victim) nodes $s,t\in \V$, and a fixed GNN-based link prediction model $f$, such that $(t,s)\notin \edges \wedge f(\h_t,\h_s)=0$, we can compute the following (instance-level) loss function:
% \begin{equation}
%     \label{eq:instance-loss}
%     \Loss(P; \G', s, t, \params) = \alpha \ladv[(f(\h_t, \h_s; \params), f(\h_t, \pi(\h_s; P);\params)] + \beta \ldist(\h_s, \pi(\h_s; P)) + \gamma \lnew(\Vnew)
% \end{equation}
% \begin{equation}
%     \label{eq:instance-loss}
%     \Loss(P; \G', s, t, \params) = \alpha \ladv[f(\h_t, \pi(\h_s; P);\params)] + \beta \ldist[\h_s, \pi(\h_s; P)] + \gamma \lnew(\Vnew)
% \end{equation}
\begin{equation}
    \label{eq:instance-loss}
    \Loss(P) = \ladv[f(\h_t, \advh_{s;P})] + \beta \ldist(\h_s, \advh_{s;P}) + \gamma \lnew(\bm{v}^{\text{new}})
\end{equation}
% \gabri{Non mi convince ancora del tutto la formulazione della loss che formalmente (e correttamente!) dipende solo da $P$, salvo poi contenere anche un termine ($\lnew$) che dipende da $\Vnew$! Non saprei, però, come riuscire a integrare tutto dentro $P$... ogni suggerimento è ben accetto! :)}
The first component ($\ladv$) penalizes when the adversarial prediction goal is {\em not} satisfied and can be computed as:
% \begin{equation}
% \label{eq:lpred}
% \ladv[f(\h_t, \pi(\h_s;P);\params)] = - \log[f(\h_t, \pi(\h_s;P);\params)],
% \end{equation}
\begin{equation}
\label{eq:lpred2}
\ladv[f(\h_t, \advh_{s;P})] = - \log[f(\h_t, \advh_{s;P})],
\end{equation}
which corresponds to a standard binary cross-entropy, where the class label to predict is always $1$, i.e., we want to enforce the prediction of an adversarial edge between $t$ and $s$.

% Let $\mathcal{C}$ be the set of source nodes which, after applying perturbation $\pi$, do {\em not} meet the prediction goal, i.e., $\mathcal{C} = \{\h_s~|~f(\h_t, \h_s) = f(\h_t, \pi(\h_s; P))\}$.
%Thus, we can compute $\ladv$ as follows:
% \begin{equation}
% \label{eq:lpred}
% \ladv[(f(\h_t, \h_s; \params), f(\h_t, \pi(\h_s;P);\params)] = \mathbbm{1}_{\mathcal{C}}(\h_s),
% \end{equation}
% where $\mathbbm{1}_{\mathcal{C}}(\cdot)$ is the well-known indicator function:
% \[
% \mathbbm{1}_{\mathcal{C}}(\h_s) = 
% \begin{cases}
% 1 ,\text{ if } \h_s \in \mathcal{C}\\
% 0, \text{ otherwise}.
% \end{cases}
% \]
The second component ($\ldist$) is %any
an arbitrary distance function that discourages $\advh_{s;P}$ from being too far away from $\h_s$, namely $\advadjM_s$ must be close to the original $\adjM_s$.
For example, $\ldist(\h_s, \advh_{s;P}) = ||\adjM_s - \advadjM_s||_p$, where $||\cdot||_p$ is the $L^p$-norm. 
%\gio{vogliamo dire che anche il terzo componente è la lp norm della somma su quel vettore?}

% The third component ($\lnew$) discourages the attacker from injecting an excessive amount of vicious nodes into the original graph network. 
The third component ($\lnew$) controls the number of vicious nodes injected into the original graph network.
In practice, $\bm{v}^{\text{new}}$ is a $|\Vnew|$-dimensional binary vector (i.e., a mask) indicating the vicious nodes injected by the attacker, i.e., $\bm{v}^{\text{new}}[u] = 1$ iff node $u \in \Vnew$ has been added to the graph network, $0$ otherwise.
For example, $\lnew(\bm{v}^{\text{new}}) = ||\bm{v}^{\text{new}}||_p$. 
In this work, we set $p=1$ both for $\ldist$ and $\lnew$.

Eventually, solving the objective defined in Eq.~\ref{eq:optimal-emb} is framed into the following optimization task:
\begin{equation}
    \label{eq:opt-adv-lp}
    \advh_{s;P^*}=\argmin_{P} \Loss(P).
\end{equation}
It is worth noticing that, in this original formulation, the optimization objective defined in Eq.~\ref{eq:opt-adv-lp} is inherently discrete. 
To make it smooth, inspired by prior work~\cite{lucic2022cf,srinivas2017cvprw}, we first consider an intermediate, real-valued perturbation matrix $\hat{P}$ with entries in $(-1,1)$, obtained by applying a hyperbolic tangent transformation ($\tanh$).
Intuitively, this matrix indicates the degree of confidence of the attacker to add or remove an edge from the adjacency matrix $\adjM'$.
Thus, we can replace $P$ with $\hat{P}$ in Eq.~\ref{eq:opt-adv-lp}, and solve the objective via standard gradient-based optimization methods like stochastic gradient descent or similar.
Eventually, to obtain the discrete matrix $P$, we simply threshold the entries of $\hat{P}$ as follows:
\[
  P_{i,j} =
  \begin{cases}
    +1 & \text{if $\hat{P}_{i,j} \geq t^+$,}\\
    -1 & \text{if $\hat{P}_{i,j} \leq t^-$,}\\
    0 & \text{otherwise.}
  \end{cases}
\]
A straightforward choice for the thresholds above is: $t^+ = 0.5$ and $t^- = -0.5$.
% Se abbiamo tempo e aggiungiamo una parte di ablation study anche su queste soglie, potremmo scrivere qui una frasetta che anticipa questa analisi
Notice, though, that $P\oplus A'$ would lead to a discrete matrix $\advadjM_s$ whose entries are in the set $\{-1,0,1,2\}$, instead of $\{0,1\}$ as required.
Indeed, removing an edge that does not exist from $\edges$, will lead to an entry equals to $-1$; on the other hand, adding an edge that already exists in $\edges$ will result in an entry equals to $2$.
% To obtain the correct final perturbed matrix $\advadjM_s$, we therefore apply a $\clamp_{[0,1]}$ function to the resulting $P\oplus A'$ element-wise, i.e., $\advadjM_s[i,j] = \clamp_{[0,1]}(P_{i,j} + A'_{i,j})~\forall (i,j)$, where $\clamp_{[0,1]}(x) = \max(0,\min(x,1))$.

We therefore obtain the correct final perturbed matrix $\advadjM_s$ by applying a $\clamp_{[0,1]}$ function element-wise, i.e., $\advadjM_s[i,j] = \clamp_{[0,1]}(P_{i,j} + A'_{i,j})~\forall (i,j)$, where $\clamp_{[0,1]}(x) = \max(0,\min(x,1))$.

%\gabri{Ho spostato il discorso sulla tecnica di ``smoothing'' della matrice di perturbazione $P$ dopo la definizione del problema di ottimizzazione (Eq.~8). In questo modo, è più comodo spiegare il motivo per cui si usano quelle trasformazioni ($\tanh + \clamp$). Inoltre, ci potrebbe essere utile per anticipare e motivare l'ablation study che avete eseguito (sia nel caso in cui decidessimo di inserirlo nel main body del paper, sia che si sposti nel supplementary).}

==> AAAI 2023 SAVAGE --_ ARXIV/sections/problem.tex <==
\section{Problem Formulation}
\label{sec:problem}

\subsection{Attack Model}
\label{subsec:attack-model}
We consider a snapshot of a network, modeled as a {\em directed} graph $\graph$, and a trained GNN-based link prediction model $f$. 
In our attack model, we assume the existence of an attacker node ($s\in \V$) that can perturb the original graph $\G$ into $\advG = (\V', \edges')$.
The perturbation represents the capability of the attacker to add a set of new vicious nodes $\Vnew$ to $\G$, such that $\V'=\V \cup \Vnew$. Furthermore, we suppose the attacker controls a subset of the original nodes $\V^s \subseteq \V$ (trivially, $s\in \V^s)$ and is capable of adding/removing edges starting from the set of governed nodes $\V^s \cup \Vnew$.
Let $\edges^+ \subseteq (\V^s \cup \Vnew)\times \V'$
and $\edges^- \subseteq (\V^s \cup \Vnew)\times \V'$ be the set of edges added and removed by the attacker, respectively.
Eventually, $\advG = (\V', \edges')$ denotes the final perturbed graph, where $\edges' = \edges \cup \edges^+ \setminus \edges^-$.
Thus, the goal of the attacker $s$ is to transform $\G$ into $\advG$, using the capabilities described above, to ultimately induce the link prediction model $f$ in recommending $s$ to a target victim node $t \in \V \setminus (\V^s \cup \Vnew)$, i.e., to suggest the creation of the directed edge $(t,s)$ between the victim and the attacker.
We also assume the attacker has full knowledge of $f$, i.e., we consider a {\em white-box} threat model, where the architecture and the entire set of parameters of $f$ ($\params = \left[ \params_f, \params_g \right ]$) are known and fixed~\cite{pitropakis2019csr,ren2020eng}.
Later in Section~\ref{subsec:transf}, we show that this requirement does not limit the adversary's power, as our proposed attack can be successfully transferred to disrupt other link prediction models in a {\em black-box} setting.


\subsection{Attack Framework}
\label{subsec:attack-framework}
The attacker $s$ aims to maximize the chance that the directed edge between the target victim $t$ and itself, i.e., $(t,s)$, will be amongst those predicted by $f$ while minimizing the ``malicious effort'' needed.

More formally, suppose $f$ is defined as in Eq.~\ref{eq:gnn-lp}.
To ease the notation, we will omit the parameters $\params_f$ and $\params_g$ from the equations below.
Also, let $\adjM$, $\adjM'$, and $\advadjM$ be the adjacency matrices associated with the original graph $\graph$, the intermediate graph $\G' = (\V', \edges)$, and the final perturbed graph $\advG = (\V', \edges')$, respectively. 
Thus, the problem for the attacker $s$ is to find the optimal perturbation $\advh^*_s \neq \h_s$ such that $f(\h_t, \advh^*_s)\neq f(\h_t, \h_s)$ by solving the objective below:
\begin{equation}
\label{eq:optimal-emb}
\begin{aligned}
\advh^*_s~=~& \argmax_{\advh_s} \Big\{ \big[f(\h_t, \advh_s) - f(\h_t, \h_s)\big] - d(\advh_s, \h_s) \Big\}, \\
%& \textrm{subject to:} \quad d(\advh_s, \h_s) \leq \delta,~~\delta \in \R_{>0}.
\end{aligned}
\end{equation}
where $f(\h_t, \advh_s) - f(\h_t, \h_s)$ measures the difference between the original and the adversarial link prediction, and $d$ captures the magnitude of the malicious effort used by the attacker for transforming $\h_s$ to $\advh_s$.

The generic perturbation $\advh_s = g(\advadjM_s, \X_s)$ indicates the attacker node embedding output by a trained GNN $g$, after the $1$-hop neighborhood of the nodes controlled by the attacker $\V^s \cup \Vnew$ has been modified according to its capabilities (i.e., by adding/removing edges as specified by $\edges^+$ and $\edges^-$, respectively).
%Specifically, we assume there exists a function $\pi$ that maps a node embedding $\h_s = g(\adjM_s, \X_s)$ into another one $\advh_s = g(\advadjM_s, \X_s)$. With a slight abuse of notation, we define:
Specifically, we assume there exists a function $\pi$ that works as follows:
\begin{equation}
\label{eq:pi}
    \advh_s = g(\pi(\adjM'), X_s) = g(\advadjM_s, \X_s),
\end{equation}
% \begin{equation}
% \label{eq:pi}
%     \advh_s = \pi(\h_s) = g(\pi(\adjM'), X_s) = g(\advadjM_s, \X_s),
% \end{equation}
where $\adjM'$ is the full adjacency matrix associated with the intermediate graph $\G'$, and $\advadjM_s = \pi(\adjM')$.
Notice that the perturbation applied by $\pi$ reflects the attacker's capabilities described in our attack model, i.e., it concerns {\em only} the topological structure of the neighborhood of the nodes controlled by the attacker, whereas the node feature matrices are left unaltered. 
We acknowledge that the ability to modify also the node feature matrices is an interesting direction to explore, and we plan to investigate this as future work since our framework is general enough to cover also that scenario.
Moreover, the perturbation induced by $\pi$ on $\h_s$ must not affect the embedding of the target victim node $\h_t$.
According to Eq.~\ref{eq:gnn-emb}, the hidden representation of a node $u$ produced by a given $l$-layer GNN ($\h_u$) is influenced by all the other nodes $v$ that are in the $l$-hop neighborhood of $u$, i.e., $\neigh^l(u)$. 
% \gio{secondo voi questa parte qua e' necessaria o si puo tagliare?}
Thus, to avoid that $\h_t$ is affected by $\pi$, we assume $t\notin \neigh^l(s)$ and, even strongly, $s\notin \neigh^l(t)$.

To measure the malicious effort of the attacker, the function $d$ captures the difference between the original and the perturbed attacker node embeddings.
Such a difference must consider: {\em(i)} the number of {\em additional} vicious nodes $\Vnew$ injected by the attacker to generate the intermediate augmented graph $\G'$; {\em(ii)} the distance between the original adjacency matrix $\adjM_s$ and the perturbed $\advadjM_s$ obtained from structural modifications (i.e., edge additions/deletions) of $\G'$. % as per our attack model.
%Again, since our attack model considers only structural modifications to the extended graph $\G'$, $d$ can be thought of as any . 
%Furthermore, $d$ must also take into account the number of vicious nodes $\Vnew$ injected by the attacker to generate the intermediate augmented graph $\G'$.

%\gabri{Qui forse manca un paragrafo di "raccordo" con la prossima sezione...}
%\gio{per me in realtà va anche bene così}

==> AAAI 2023 SAVAGE --_ ARXIV/sections/related.tex <==
\section{Related Work}
\label{sec:related} 
\paragraph{Link Prediction.}
Link prediction is one of the most investigated problems in modern graph analysis.
One class of simple yet effective approaches for link prediction is called heuristic methods.
These assume that the existence of a link between two nodes depends on their ``similarity''. 
In practice, they use some predefined heuristics to compute node similarity scores as the link probability~\cite{liben2003cikm,lu2011link}.
% Existing heuristics can be categorized based on the maximum hop of neighbors needed to calculate the node similarity score.
% For example, common neighbors~\cite{newman2001clustering}, Jaccard~\cite{liben2003cikm}, and preferential attachment~\cite{barabasi1999pa} are first-order
% heuristics, since they only involve the one-hop neighbors of two target nodes. 
% Adamic-Adar~\cite{adamic2003sn} and resource allocation~\cite{zhou2009predicting} are second-order heuristics, as they consider up to the two-hop neighborhood of the target nodes.
% There are also some high-order heuristics that require knowing the entire network. Examples include Katz index~\cite{katz1953new}, rooted PageRank~\cite{brin1998pagerank}, and SimRank~\cite{jeh2002simrank}.
% VERSIONE BREVE:
Popular heuristics include: Common Neighbors~\cite{newman2001clustering}, Jaccard~\cite{liben2003cikm}, Preferential Attachment~\cite{barabasi1999pa}, Adamic-Adar~\cite{adamic2003sn}, Resource Allocation~\cite{zhou2009predicting}, Katz~\cite{katz1953new}, PageRank~\cite{brin1998pagerank}, and SimRank~\cite{jeh2002simrank}.

Although working well in practice, heuristic methods have strong ``hand-coded'' assumptions on when links may exist.
To overcome this limitation, the link prediction problem has been formulated as a standard binary classification task and solved using well-known supervised learning techniques~\cite{alhasan2006sdm}.
%, such as decision trees, support vector machines, k-nearest neighbors, multilayer perceptrons, and different ensembles of these classifiers~\cite{alhasan2006sdm}. 

With the advancements of deep learning and, specifically, graph neural networks (GNNs), several approaches have recently proposed effective GNN-based link prediction methods~\cite{zhang2018neurips,li2021icml}.
Roughly speaking, GNNs allow to learn suitable representations (i.e., embeddings) of graph nodes by aggregating information derived from the local neighborhood of each individual node.
These node embeddings are in turn used as input of a downstream link prediction function, thus making the whole model's architecture end-to-end trainable. 
In this work, we focus on a specific attack to GNN-based link prediction.

For a comprehensive survey on link prediction, we refer the reader to~\cite{martinez2016cs,kumar2020link,wu2020comprehensive}.

% Lately, researchers have introduced graph embedding algorithms for the problem of link prediction.
% In this setting, a mapping function is responsible for projecting the features of all nodes into a lower (or higher, for that matter) dimensional latent space.
% DeepWalk \cite{perozzi2014deepwalk}, and later node2vec \cite{grover2016node2vec} are the most important methods in this regard. However, while considering the topology of the graph, these methods fail to take into account the feature information of nodes.



% Kipf and Welling \cite{kipf2016semi}, proposed graph convolutional network (GCN) for semi-supervised embedding learning. 
% This method learns hidden node representation based on a message-passing algorithm, in their case, a simple average over neighboring nodes, interleaved with deep embedding of their features.
% They later formulated GAE \cite{kipf2016variational}, which uses two graph convolutional layers to capture the information of graph structure and node features at the same time and designs a decoder to represent the node relational information from their embeddings by reconstructing the graph adjacency matrix. 
% These formulation, and the ones that later followed \cite{velivckovic2017graph} \cite{ying2021transformers} \cite{wu2020comprehensive} \cite{bronstein2017geometric}, achieved much higher performance for the task of link prediction.

\paragraph{Adversarial Attacks to Link Prediction.}
% Adversarial attacks on neural networks have been first popularized by Goodfellow \cite{goodfellow2014explaining}. Here, he crafted a seemingly random perturbation to the original image that could fool a CNN-based model into classifying a panda as a Gibbon. However, this perturbation was not random but was crafted using gradient information. Many works followed on other architectures, such as RNN, and most notably for our application, GNN.
Although very powerful, studies have shown that machine learning models may be vulnerable to so-called {\em adversarial attacks}, i.e., carefully crafted malicious examples designed to fool the predictive models. 
Typically, these adversarial inputs are generated by introducing minor -- yet thoughtfully selected -- perturbations to regular inputs. 
These attacks have been widely proven successful in many critical domains, such as image recognition~\cite{goodfellow2014explaining} and malware detection~\cite{grosse2017esorics}.
However, a few works have explored how effective such adversarial attacks may be for link prediction algorithms, especially those based on GNNs, which require the attacker to perturb the input graph. 
Amongst these studies, it is worth mentioning~\cite{zugner2018adversarial, chen2020link,lin2020adversarial}. We refer the reader to~\cite{dai2022comprehensive} for a comprehensive survey.

%\paragraph{Adversarial Attacks by Injection of Vicious Nodes.}
The methods above assume that the attacker can control a subset of existing nodes. As stated in Section~\ref{sec:intro}, though, this is a pretty unrealistic premise, as it would be prohibitively expensive. 
To address this issue,~\cite{wang2018attack} introduce the capability for the attacker to generate {\em new} (i.e., fake/vicious) nodes to mount the attack more efficiently.
Furthermore,~\cite{wang2020scalable} propose a linear approximation of the previous method to make it more scalable. 
%Dai {\em et al}.~
\citet{dai2022targeted} formulate a universal perturbation that can target multiple nodes and still remain effective. 

In both classic and vicious settings, all the methods presented so far introduce an unnoticeability constraint of the graph perturbation. This constraint is usually of two kinds: either the attacker is given a fixed budget to spend~\cite{chen2020link}, or some rules are imposed to control the difference between the original and the perturbed graph, like in~\cite{lin2020adversarial}.
Either way, this is treated as an upper bound on the amount of ``malicious resources'' used to implement the attack and does not promote frugality. 
In fact, the adversary typically saturates the constraint to ensure that the attack is successful.
On the other hand, the method we propose in this work enforces the sparsity of the malicious resources used by the attacker (see Fig.~\ref{fig:teaser}).
% HO TOLTO QUESTO CHE NON MI SEMBRAVA TROPPO UTILE QUI:
%Furthermore, different from existing methods, our technique can effectively solve this issue through a suitable set of transformations on the perturbation matrix, partially inspired by~\cite{lucic2022cf}.


==> AAAI 2023 SAVAGE --_ ARXIV/tables/ablation_X.tex <==
\begin{table}[h]
\centering
\caption{\label{tab:abl_X} bla bla}
\begin{tabular}{llllll}
\hline
Method & AR & AP & OP & AN & AE \\ \hline
Mean   &    &    &    &    &    \\
Median &    &    &    &    &    \\
Rand   &    &    &    &    &    \\
Ones   &    &    &    &    &    \\
Zeros  &    &    &    &    &    \\
Rand E &    &    &    &    &    \\ \hline
\end{tabular}
\end{table}

==> AAAI 2023 SAVAGE --_ ARXIV/tables/ablation_transform.tex <==
% \begin{table}[h]
% \centering
% \caption{\label{tab:abl_tr} Results for different choices of transformation. Tanh and Tanh + Clamp obtain the best results. By removing these transformations performance drops drastically. We thereby argue that our choice is sensible and necessary for this formulation.}
% \begin{tabular}{lllll}
% \toprule
% Method       & AR   & AP   & OP   & CP   \\ \midrule
% None         & 0.4  & 0.57 & 0.51 & 0.29 \\
% Tanh         & 0.55 & 0.62 & 0.51 & 0.61 \\
% Clamp        & 0.2  & 0.55 & 0.51 & 0.22 \\
% Tanh + Clamp & 0.55 & 0.62 & 0.51 & 0.51 \\ \midrule
% A No Clamp   & 0.05 & 0.49 & 0.51 & 1    \\ \midrule
% \end{tabular}
% \end{table}

\begin{table*}[h]
    \begin{minipage}{.45\linewidth}
    \centering
    \caption{\label{tab:abl_tr} Results for different choices of transformation. $\tanh$ and $\tanh$ + $\clamp$  obtain the best results. By removing these transformations performance drops drastically. We thereby argue that our choice is sensible and necessary for this formulation.}
        \begin{tabular}{lllll}
        \toprule
        Method       & AR   & AP   & OP   & CP   \\ \midrule
        {\em none}         & 0.40  & 0.57 & 0.51 & 0.29 \\
        $\tanh$         & 0.55 & 0.62 & 0.51 & 0.61 \\
        $\clamp$        & 0.20  & 0.55 & 0.51 & 0.22 \\
        $\tanh$ + $\clamp$ & 0.55 & 0.62 & 0.51 & 0.51 \\ \midrule
        A No $\clamp$   & 0.05 & 0.49 & 0.51 & 1    \\ \midrule
        \end{tabular}
    \end{minipage}%
    \hspace{0.05\linewidth}
    % 
    % \hfill
    % \parbox{.45\linewidth}{
    % \centering
    % 
    % \vspace{-12.9em}
    \begin{minipage}{.5\linewidth}
    \centering
    \caption{\label{tab:tra_alg} Scores for popular link predictions heuristics. All scores were zero  for the unperturbed version of the model. We argue this showcases the transferability of our attack.}
        \begin{tabular}{cc}
        \toprule
        Algorithm & Score   \\\midrule
        Common Neighbors & \\
        Jaccard & \\
        Preference Attachment & \\
        Adam-Adar & \\
        Resource Allocation & \\
        Katz Index \cite{katz1953new} & 0.15\\
        PageRank \cite{BRIN1998107} &  0.17\\
        SimRank \cite{10.1145/775047.775126} & 0.65\\
        \bottomrule
    \end{tabular}
    \end{minipage}
    % }
\end{table*}



==> AAAI 2023 SAVAGE --_ ARXIV/tables/main_results_fake_data.tex <==
\begin{table*}[h]
\centering
\caption{\label{tab:main_results_fake} bla bla}
\begin{tabular}{llllll}
\cline{2-6}
              & \multicolumn{5}{c}{\textbf{Synthetic Data}} \\ \cline{2-6} 
Method        & AR      & AP     & OP     & AN     & AE     \\ \hline
Source        &         &        &        &        &        \\
Source L      &         &        &        &        &        \\
VN            &         &        &        &        &        \\
VN L          &         &        &        &        &        \\
Source + VN   &         &        &        &        &        \\
Source + VN L &         &        &        &        &        \\ \hline
\end{tabular}
\end{table*}

==> AAAI 2023 SAVAGE --_ ARXIV/tables/main_results_real_data.tex <==
\begin{table*}[h]
\centering
\caption{\label{tab:main_result_real}bla bla}
\begin{tabular}{lllllllllll}
\cline{2-11}
              & \multicolumn{5}{c}{\textbf{OGB - Arxiv}} & \multicolumn{5}{c}{\textbf{OGB - Citation 2}} \\ \cline{2-11} 
Method        & AR     & AP     & OP     & AN    & AE    & AR      & AP      & OP      & AN     & AE     \\ \midrule
Source        &        &        &        &       &       &         &         &         &        &        \\
Source L      &        &        &        &       &       &         &         &         &        &        \\
VN            &        &        &        &       &       &         &         &         &        &        \\
VN L          &        &        &        &       &       &         &         &         &        &        \\
Source + VN   &        &        &        &       &       &         &         &         &        &        \\
Source + VN L &        &        &        &       &       &         &         &         &        &        \\ \midrule
\end{tabular}

\end{table*}

==> AAAI 2023 SAVAGE --_ ARXIV/tables/s_svn_table.tex <==
\begin{table*}[]
\centering
\caption{\label{tab:s_svn_result}Results on several datasets for the loss penalized, and not, version. We achieve comparable results by using only a fraction of the resources.}
\begin{tabular}{lllllllllllll}
\toprule
                & \multicolumn{4}{c}{\textbf{Twitter}} & \multicolumn{4}{c}{\textbf{GPlus}} & \multicolumn{4}{c}{\textbf{Citation2}}\\ \cmidrule(lr){2-5}\cmidrule(lr){6-9}\cmidrule(lr){10-13}
Method          & AR & AN & MFP & KL & AR    & AN   & MFP  & KL & AR & AN & MFP & KL \\ \midrule
{\em OUR}       &    &    &     &    & 0.93  & 46.7 & 0.90 &    &    &    &     &    \\    
{\em OUR I}     &    &    &     &    & 0.97  & 50.0   & 0.95 &    &    &    &     &    \\ 
{\em OUR L}     &    &    &     &    & 0.80  & 35.7 & 0.79 &    &    &    &     &    \\ 
{\em OUR IL}    &    &    &     &    & 0.97  & 38.7 & 0.95 &    &    &    &     &    \\ 
{\em Random L}  &    &    &     &    &       &      &      &    &    &    &     &    \\ 
{\em Random H}  &    &    &     &    &       &      &      &    &    &    &     &    \\ 
{\em AIGA}      &    &    &     &    & 0.23  & 50   & 0.29 &    &    &    &     &    \\ \midrule
\end{tabular}

\end{table*}

==> AAAI 2023 SAVAGE --_ ARXIV/tables/transferability_alg.tex <==
% \begin{table}[]
% \centering
%     \caption{\label{tab:tra_alg} bla bla}
%         \begin{tabular}{ccc}
%         \hline
%         Algorithm       & Formula & Score   \\\hline
%          & & &\\
%         Katz Index \cite{katz1953new}        & $\sum_{l=1}^{\infty} \beta^l | path(x, y) = l|$ & \\
%          & & &\\
%         PageRank \cite{BRIN1998107}         & $q_{xy} + q_{yx}$ &\\
%          & & &\\
%         SimRank \cite{10.1145/775047.775126}         & $\gamma \frac{\sum_{a \in \Gamma(x)} \sum_{b \in \Gamma(y)} score(a, b)}{|\Gamma(x)| \times |\Gamma(y)|}$ &\\
%         & & &\\\hline
%     \end{tabular}
% \end{table}

\begin{table}[htbp]
% \vspace{-0.5mm}
\centering
\small
% Remove this for undo column width
\addtolength{\tabcolsep}{-8pt}
\caption{\label{tab:tra_alg} Lift scores for popular link prediction heuristics before and after being attacked by \savag. 
Given the large increase in heuristic values after the attack, we claim that our attacks successfully transfer to different black-box methods.
}
    \begin{tabular}{cc}
    \toprule
    Heuristic & \begin{tabular}[c]{@{}c@{}}Lift Score \\ (attack/non-attack)\end{tabular} \\\midrule
    Common Neighbors~\cite{newman2001clustering} & $70 \times$\\
    Jaccard~\cite{liben2003cikm} & $93\times$\\
    Preference Attachment~\cite{barabasi1999pa} & $3.4\times$\\
    Adam-Adar~\cite{adamic2003friends} & $61\times$\\
    Resource Allocation~\cite{zhou2009predicting} & $2.9\times$\\
    Katz Index~\cite{katz1953new} & $3 e5\times$\\
    PageRank~\cite{brin1998pagerank} &  $1.2\times$\\
    SimRank~\cite{jeh2002simrank} & $20\times$\\
    \bottomrule
    \end{tabular}

\end{table} 
    

% \begin{table}[htbp]
% \caption{\label{tab:tra_alg} Scores for popular link predictions heuristics. Given the large increase between its unperturbed and its perturbed version, we claim that our attacks successfully transfer to different, unobserved, settings.}
% \begin{tabular}{@{}ccccc@{}}
% \toprule
% Algorithm & Random & AIGA & SAVAGE1 & SAVAGE2 \\ \midrule
% \begin{tabular}[c]{@{}c@{}}Common \\ Neighbors\end{tabular} & $70\%$ & $70\%$ & $70\%$ & $70\%$ \\ \midrule
% Jaccard & $93\%$ & $93\%$ & $93\%$ & $93\%$ \\ \midrule
% \begin{tabular}[c]{@{}c@{}}Preference \\ Attachment\end{tabular} & $3.40\%$ & $3.40\%$ & $3.40\%$ & $3.40\%$ \\ \midrule
% Adam-Adar & $61\%$ & $61\%$ & $61\%$ & $61\%$ \\ \midrule
% \begin{tabular}[c]{@{}c@{}}Resource \\ Allocation\end{tabular} & $2.9\%$ & $2.9\%$ & $2.9\%$ & $2.9\%$ \\ \midrule
% Katz Index & $2.80$ & $2.80$ & $2.80$ & $2.80$ \\ \midrule
% PageRank & $1.23\%$ & $1.23\%$ & $1.23\%$ & $1.23\%$ \\ \midrule
% SimRank & $20\%$ & $20\%$ & $20\%$ & $20\%$ \\ \bottomrule
% \end{tabular}
% \end{table}

==> AAAI 2023 SAVAGE --_ ARXIV/tables/vn_table.tex <==
\begin{table*}[htbp]
\vspace{-4mm}
\small
% Remove this for undo column width
\addtolength{\tabcolsep}{-3pt}

\centering

\centering
\caption{\label{tab:vn_result} 
We report several metrics regarding the effectiveness and efficacy of \savag. First, we manage to mount very effective link prediction attacks. Second, thanks to our penalized framework, we are able to greatly reduce the amount of vicious nodes required. KL is in reported in base $10^{-3}.$
% Effectiveness and efficiency of link prediction attacks generated with \savag\ (KL is in reported in base $10^{-3}$).
}

\begin{tabular}{lllllllllllll}

\toprule
                & \multicolumn{4}{c}{\textit{Twitter}} & \multicolumn{4}{c}{\textit{GPlus}} & \multicolumn{4}{c}{\textit{Citation2}}\\ \cmidrule(lr){2-5}\cmidrule(lr){6-9}\cmidrule(lr){10-13}
Method          & AR $\uparrow$ & AN $\downarrow$ & AP $\uparrow$ & KL $\downarrow$ & AR $\uparrow$ & AN $\downarrow$ & AP $\uparrow$ & KL $\downarrow$ & AR $\uparrow$ & AN $\downarrow$ & AP $\uparrow$ & KL $\downarrow$ \\ \midrule
\savag    & $0.75$ & $\mathbf{57.95}$  & $0.73$ & $3.00$ & $0.80$ & $\mathbf{35.70}$ & $0.79$ & $0.03$ & $0.85$ & $13.10$ & $0.87$ & $1.00$   \\ 
\savag-I    & $0.75$ & $61.05$  & $0.70$ & $3.00$ & $\mathbf{0.97}$ & $38.70$ & $\mathbf{0.95}$ & $0.03$ & $\mathbf{1.00}$ & $\mathbf{7.05}$  & $0.98$ & $0.30$   \\
\savag-N       & $0.95$ & $95.30$  & $0.93$ & $4.00$ & $0.93$ & $46.70$ & $0.90$ & $1.00$ & $0.85$ & $37.70$ & $0.89$ & $4.00$   \\    
\savag-NI     & $\mathbf{1.00}$ & $95.55$  & $\mathbf{0.99}$ & $4.00$ & $\mathbf{0.97}$ & $50.00$ & $\mathbf{0.95}$ & $0.03$ & $\mathbf{1.00}$ & $47.10$ & $\mathbf{0.99}$ & $3.00$   \\ 
AIGA      & $0.60$ & $100.0$ & $0.61$ & $\mathbf{0.00}$             & $0.23$ & $50.00$ & $0.29$ & $\mathbf{0.00}$             & $0.90$ & $50.00$ & $0.93$ & $\mathbf{0.03}$ \\ \midrule
 RAND-L  & $0.00$ & $23.15$  & $0.04$ & $5.00$ & $0.00$ & $13.70$ & $0.04$ & $1.00$ &  $0.05$      & $12.95$        & $0.03$        & $6.00$ \\ 
RAND-H  & $0.10$ & $74.70$  & $0.11$ & $10.00$ & $0.00$ & $37.35$ & $0.06$ & $10.00$ &  $0.00$      & $38.85$         & $0.03$        & $10.00$ \\ \midrule 
\end{tabular}


\vspace{1mm}


\begin{tabular}{lllllllllllllllll}
\toprule
                & \multicolumn{4}{c}{\textit{Arxiv}} & \multicolumn{4}{c}{\textit{Cora}} & \multicolumn{4}{c}{\textit{Wiki}} & \multicolumn{4}{c}{\textit{Synthetic}}\\ \cmidrule(lr){2-5}\cmidrule(lr){6-9}\cmidrule(lr){10-13}\cmidrule(lr){14-17}
Method          & AR $\uparrow$ & AN $\downarrow$ & AP $\uparrow$ & KL $\downarrow$ & AR $\uparrow$ & AN $\downarrow$ & AP $\uparrow$ & KL $\downarrow$ & AR $\uparrow$ & AN $\downarrow$ & AP $\uparrow$ & KL $\downarrow$ & AR $\uparrow$ & AN $\downarrow$ & AP $\uparrow$ & KL $\downarrow$ \\ \midrule
\savag     & $0.80$ & $35.70$ & $0.80$ & $5.00$ & $0.83$ & $47.60$ & $0.83$ & $1.00$ & $\mathbf{1.00}$ & $14.20$ & $0.88$ & $7.00$ & $\mathbf{1.00}$ & $14.00$ & $0.88$ & $7.00$   \\ 
\savag-I  & $0.75$ & $\mathbf{34.90}$ & $0.75$ & $5.00$ & $\mathbf{0.96}$ & $\mathbf{33.60}$ & $\mathbf{0.97}$ & $\mathbf{0.04}$ & $0.60$ & $\mathbf{10.25}$ & $0.63$ & $3.00$ & $0.60$ & $\mathbf{9.00}$ & $0.63$ & $3.00$\\
\savag-N       & $\mathbf{0.95}$ & $44.55$ & $\mathbf{0.93}$ & $5.00$ & $0.83$ & $59.80$ & $0.83$ & $3.00$ & $\mathbf{1.00}$ & $29.70$ & $\mathbf{0.96}$ & $7.00$ & $\mathbf{1.00}$ & $29.00$ & $\mathbf{0.96}$ & $7.00$   \\    
\savag-NI     & $0.90$ & $43.05$ & $0.89$ & $5.00$ & $0.70$ & $49.40$ & $0.69$ & $3.00$ & $0.70$ & $11.10$ & $0.68$ & $3.00$ & $0.70$ & $11.00$ & $0.68$ & $3.00$   \\ 
AIGA      & $0.70$ & $50.00$ & $0.67$ & $\mathbf{0.00}$                & $0.80$ & $80.00$   & $0.79$ & $0.40$ & $0.40$ & $50.00$   & $0.47$ & $\mathbf{0.00}$                & $0.90$ & $50.00$ & $0.93$ & $\mathbf{0.03}$   \\ \midrule
RAND-L  & $0.10$ & $11.40$ & $0.11$ & $6.00$ & $0.00$ & $17.50$         & $0.00$     &    $4.00$              & $0.10$     & $13.10$     & $0.29$      & $3.00$ & $0.10$    & $13.10$ & $0.31$ & $6.00$ \\ 
RAND-H  & $0.15$ & $37.70$ & $0.14$ & $10.00$ & $0.00$     & $60.15$     & $0.00$     & $10.00$  & $0.05$     & $36.65$     & $0.29$      & $10.00$  & $0.10$    & $37.40$   & $0.22$ &$30.00$ \\ \bottomrule
\end{tabular}

\end{table*}

==> AAAI 2023 SAVAGE --_ ARXIV/tikz/abl_betas.tex <==
\begin{tikzpicture}%[width=\textwidth]
\begin{axis}[
    title={Ablation Study on $\beta$},
    xlabel={$\beta$},
    ylabel={Nodes Used},
    xmin=0, xmax=10,
    ymin=0, ymax=15,
    xtick={},
    ytick={},
    legend pos=north west,
    ymajorgrids=true,
    grid style=dashed,
]
\addplot[
    color=blue,
    mark=square,
    ]
    coordinates {
    (0, 14.85)
    (1, 7.6)
    (2, 5)
    (3, 3.5)
    (4, 2.95)
    (5, 2.6)
    (6, 2.15)
    (7, 2)
    (8, 1.7)
    (9, 1.55)
    (10, 1.5)
    };
    % \legend{Nodes Used}
\end{axis}
\end{tikzpicture}%
\caption{Amount of resources used at the variying of the penalty loss $\beta$. It can be noticed how the decrease in the resources used produces a well behaved monotonic curve.}
    

==> AAAI 2023 SAVAGE --_ ARXIV/tikz/abl_gammas.tex <==
\begin{tikzpicture}%[width=\textwidth]
\begin{axis}[
    title={Ablation Study on $\gamma$},
    xlabel={$\gamma$},
    ylabel={log(Nodes Used)},
    xmin=0, xmax=10,
    ymin=-2.5, ymax=4,
    xtick={},
    ytick={},
    legend pos=north west,
    ymajorgrids=true,
    grid style=dashed,
]
\addplot[
    color=blue,
    mark=square,
    ]
    coordinates {
    (0, 3.18)
    (1, 0.97)
    (2, 0.44)
    (3, 0.05)
    (4, 0.05)
    (5, -0.51)
    (6, -0.6)
    (7, -0.7)
    (8, -1.6)
    (9, -1.05)
    (10, -1.9)
    };
    % \legend{Nodes Used}
\end{axis}
\end{tikzpicture}%
\caption{Amount of resources used (log-scale) at the variying of the penalty loss $\gamma$. Again, it can be noticed how the decrease in the resources used produces a well behaved, almost monotonic, curve.}
% (0, 24.25)
%     (1, 2.65)
%     (2, 1.55)
%     (3, 1.05)
%     (4, 1.05)
%     (5, 0.6)
%     (6, 0.55)
%     (7, 0.5)
%     (8, 0.2)
%     (9, 0.35)
%     (10, 0.15)

==> tables/ablation_X.tex <==
\begin{table}[h]
\centering
\caption{\label{tab:abl_X} bla bla}
\begin{tabular}{llllll}
\hline
Method & AR & AP & OP & AN & AE \\ \hline
Mean   &    &    &    &    &    \\
Median &    &    &    &    &    \\
Rand   &    &    &    &    &    \\
Ones   &    &    &    &    &    \\
Zeros  &    &    &    &    &    \\
Rand E &    &    &    &    &    \\ \hline
\end{tabular}
\end{table}

==> tables/ablation_transform.tex <==
% \begin{table}[h]
% \centering
% \caption{\label{tab:abl_tr} Results for different choices of transformation. Tanh and Tanh + Clamp obtain the best results. By removing these transformations performance drops drastically. We thereby argue that our choice is sensible and necessary for this formulation.}
% \begin{tabular}{lllll}
% \toprule
% Method       & AR   & AP   & OP   & CP   \\ \midrule
% None         & 0.4  & 0.57 & 0.51 & 0.29 \\
% Tanh         & 0.55 & 0.62 & 0.51 & 0.61 \\
% Clamp        & 0.2  & 0.55 & 0.51 & 0.22 \\
% Tanh + Clamp & 0.55 & 0.62 & 0.51 & 0.51 \\ \midrule
% A No Clamp   & 0.05 & 0.49 & 0.51 & 1    \\ \midrule
% \end{tabular}
% \end{table}

\begin{table*}[h]
    \begin{minipage}{.45\linewidth}
    \centering
    \caption{\label{tab:abl_tr} Results for different choices of transformation. $\tanh$ and $\tanh$ + $\clamp$  obtain the best results. By removing these transformations performance drops drastically. We thereby argue that our choice is sensible and necessary for this formulation.}
        \begin{tabular}{lllll}
        \toprule
        Method       & AR   & AP   & OP   & CP   \\ \midrule
        {\em none}         & 0.40  & 0.57 & 0.51 & 0.29 \\
        $\tanh$         & 0.55 & 0.62 & 0.51 & 0.61 \\
        $\clamp$        & 0.20  & 0.55 & 0.51 & 0.22 \\
        $\tanh$ + $\clamp$ & 0.55 & 0.62 & 0.51 & 0.51 \\ \midrule
        A No $\clamp$   & 0.05 & 0.49 & 0.51 & 1    \\ \midrule
        \end{tabular}
    \end{minipage}%
    \hspace{0.05\linewidth}
    % 
    % \hfill
    % \parbox{.45\linewidth}{
    % \centering
    % 
    % \vspace{-12.9em}
    \begin{minipage}{.5\linewidth}
    \centering
    \caption{\label{tab:tra_alg} Scores for popular link predictions heuristics. All scores were zero  for the unperturbed version of the model. We argue this showcases the transferability of our attack.}
        \begin{tabular}{cc}
        \toprule
        Algorithm & Score   \\\midrule
        Common Neighbors & \\
        Jaccard & \\
        Preference Attachment & \\
        Adam-Adar & \\
        Resource Allocation & \\
        Katz Index \cite{katz1953new} & 0.15\\
        PageRank \cite{BRIN1998107} &  0.17\\
        SimRank \cite{10.1145/775047.775126} & 0.65\\
        \bottomrule
    \end{tabular}
    \end{minipage}
    % }
\end{table*}



==> tables/main_results_fake_data.tex <==
\begin{table*}[h]
\centering
\caption{\label{tab:main_results_fake} bla bla}
\begin{tabular}{llllll}
\cline{2-6}
              & \multicolumn{5}{c}{\textbf{Synthetic Data}} \\ \cline{2-6} 
Method        & AR      & AP     & OP     & AN     & AE     \\ \hline
Source        &         &        &        &        &        \\
Source L      &         &        &        &        &        \\
VN            &         &        &        &        &        \\
VN L          &         &        &        &        &        \\
Source + VN   &         &        &        &        &        \\
Source + VN L &         &        &        &        &        \\ \hline
\end{tabular}
\end{table*}

==> tables/main_results_real_data.tex <==
\begin{table*}[h]
\centering
\caption{\label{tab:main_result_real}bla bla}
\begin{tabular}{lllllllllll}
\cline{2-11}
              & \multicolumn{5}{c}{\textbf{OGB - Arxiv}} & \multicolumn{5}{c}{\textbf{OGB - Citation 2}} \\ \cline{2-11} 
Method        & AR     & AP     & OP     & AN    & AE    & AR      & AP      & OP      & AN     & AE     \\ \midrule
Source        &        &        &        &       &       &         &         &         &        &        \\
Source L      &        &        &        &       &       &         &         &         &        &        \\
VN            &        &        &        &       &       &         &         &         &        &        \\
VN L          &        &        &        &       &       &         &         &         &        &        \\
Source + VN   &        &        &        &       &       &         &         &         &        &        \\
Source + VN L &        &        &        &       &       &         &         &         &        &        \\ \midrule
\end{tabular}

\end{table*}

==> tables/s_svn_table.tex <==
\begin{table*}[]
\centering
\caption{\label{tab:s_svn_result}Results on several datasets for the loss penalized, and not, version. We achieve comparable results by using only a fraction of the resources.}
\begin{tabular}{lllllllllllll}
\toprule
                & \multicolumn{4}{c}{\textbf{Twitter}} & \multicolumn{4}{c}{\textbf{GPlus}} & \multicolumn{4}{c}{\textbf{Citation2}}\\ \cmidrule(lr){2-5}\cmidrule(lr){6-9}\cmidrule(lr){10-13}
Method          & AR & AN & MFP & KL & AR    & AN   & MFP  & KL & AR & AN & MFP & KL \\ \midrule
{\em OUR}       &    &    &     &    & 0.93  & 46.7 & 0.90 &    &    &    &     &    \\    
{\em OUR I}     &    &    &     &    & 0.97  & 50.0   & 0.95 &    &    &    &     &    \\ 
{\em OUR L}     &    &    &     &    & 0.80  & 35.7 & 0.79 &    &    &    &     &    \\ 
{\em OUR IL}    &    &    &     &    & 0.97  & 38.7 & 0.95 &    &    &    &     &    \\ 
{\em Random L}  &    &    &     &    &       &      &      &    &    &    &     &    \\ 
{\em Random H}  &    &    &     &    &       &      &      &    &    &    &     &    \\ 
{\em AIGA}      &    &    &     &    & 0.23  & 50   & 0.29 &    &    &    &     &    \\ \midrule
\end{tabular}

\end{table*}
